GBTX emulator for development and special versions of GBT-based readout chains

The GBTX ASIC is a standard solution for providing fast control and data readout for radiation detectors used in HEP experiments. However, it is subject to export control restrictions due to the usage of radiation-hard technology. An FPGA-based GBTX emulator (GBTxEMU) has been developed to enable the development of GBT-based readout chains in countries where the original GBTX cannot be imported. Thanks to utilizing a slightly modified GBT-FGPA core, it maintains basic compatibility with standard GBT-based systems. The GBTxEMU also may be an interesting solution for developing GBT-based readout chains for less demanding experiments.

==> emu_old.tex <==
The GBTX ASIC is a standard solution for providing fast control and data readout for radiation detectors used in HEP experiments [1,2]. However, it is subject to export control restrictions due to the usage of radiation-hard technology. To enable the development of GBT-based readout chains in countries, where the original GBTX can’t be imported, an FPGA-based GBTX emulator (GBTxEMU) has been developed. Thanks to utilization of slightly modified GBT-FGPA core [3] it maintains basic compatibility with standard GBT-based systems.
The emulator may be implemented in a relatively cheap Artix 7 FPGA chip. It provides the basic functionality of the original GBTX - time-deterministic transport of downlink messages, allowing synchronization and fast control of front-end, and high-speed transmission of hit data in the uplink direction. The GBTxEMU supports limited modes of E-Link operation with a clock frequency of 40 or 80 MHz. The downlink operates with SDR (40 or 80 Mbps) and the uplink with DDR (80 or 160 Mbps). The number of supported E-Links depends on the E-Link clock frequency and is equal to 28 for 80 MHz and 56 for 40 MHz. 
The emulator may also be used in special versions of the GBT-based readout chain, where radiation hardness is not essential, but the overall price of the system may be important. Currently, its usage in DAQ systems for BM@N and MPD experiments is planned [4]. The original hardware implementation is based on a commercial Artix-7 module and a dedicated baseboard providing jitter cleaner and communication interfaces. The development version was created at GSI, and the final BM@N version in Eurocard format was designed at JINR. In the applications where the maximum throughput of the GBTxEMU is not needed, the board may be placed at some distance from the on-detector electronics, outside of high magnetic field and radiation enviroment. The 10-meter length copper cable connection between the front-end electronics and GBTxEMU was proven to be stable in the BM@N STS project. 
Thanks to the FPGA-based architecture, the GBTxEMU is highly flexible. The end-user may connect his own IP blocks to the internal bus, creating additional control interfaces. A special address space management system [5] facilitates their easy integration with the control software.  The internal registers are accessible either via the GBT link or via IPbus (using 100Mbps or 1Gbps Ethernet). The embedded Forth-based CPU may perform complex initialization procedures during power-up, and be used for interactive diagnostics. 
The GBTxEMU may be an interesting solution for the development of GBT-based readout chains and for less demanding experiments.

[1]	J.Mitra et al., “Trigger and timing distributions using the TTC-PON and GBT bridge connection in ALICE for the LHC Run 3 Upgrade”, doi: 10.1016/j.nima.2018.12.076
[2]	J. Lehnert et al.,“GBT based readout in the CBM experiment”,doi:10.1088/1748-0221/12/02/C02061
[3]	M. Barros Marin, “The GBT-FPGA core: features and challenges”, doi:10.1088/1748-0221/10/03/C03021
[4]	W.M.Zabolotny et al., “GBTx emulation for BM@N/MPD data acquisition systems”, NICA Days 2019, http://cern.ch/go/J8TL
[5]	W.M.Zabolotny et al., “Automatic management of local bus address space in complex FPGA-implemented hierarchical systems”, doi: 10.1117/12.2536259

The work has been partially supported by GSI, and partially by the statutory funds of Institute of Electronic Systems. This project has also received funding from the European Union’s Horizon 2020 research and innovation programme under grant agreement No 871072.



==> smietnik.tex <==

\begin{figure}[htbp]
	\centering %
	\includegraphics[width=.4\textwidth]{rysunki/EMUv0_GSI}
	%
	%
	\caption{\label{fig:i} and EMUv0\_GSI.}
\end{figure}

\begin{figure}[htbp]
	\centering %
	\includegraphics[width=.6\textwidth]{rysunki/EMUv0b_GSI}
	%
	%
	\caption{\label{fig:i1} EMUv0b\_GSI.}
\end{figure}


\begin{figure}[htbp]
	\centering %
	\includegraphics[width=.6\textwidth]{rysunki/IMG-20190624-WA0000}
	%
	%
	\caption{\label{fig:i7} IMG-20190624-WA0000.}
\end{figure}

\begin{figure}[htbp]
	\centering %
	\includegraphics[width=.6\textwidth]{rysunki/IMG-20191008-WA0003}
	%
	%
	\caption{\label{fig:i8} IMG-20191008-WA0003.}
\end{figure}

\begin{figure}[htbp]
	\centering %
	\includegraphics[width=.6\textwidth]{rysunki/gbtxemu}
	%
	%
	\caption{\label{fig:i9} gbtxemu.}
\end{figure}

\begin{figure}[htbp]
	\centering %
	\includegraphics[width=.6\textwidth]{rysunki/photo}
	%
	%
	\caption{\label{fig:i10} photo.}
\end{figure}


\begin{figure}[htbp]
	\centering %
	\includegraphics[width=.6\textwidth]{rysunki/photo3}
	%
	%
	\caption{\label{fig:i12} photo3.}
\end{figure}



